CLIP4STR: A Simple Baseline for Scene Text Recognition with Pre-trained Vision-Language Model

Pre-trained vision-language models~(VLMs) are the de-facto foundation models for various downstream tasks. However, scene text recognition methods still prefer backbones pre-trained on a single modality, namely, the visual modality, despite the potential of VLMs to serve as powerful scene text readers. For example, CLIP can robustly identify regular (horizontal) and irregular (rotated, curved, blurred, or occluded) text in images. With such merits, we transform CLIP into a scene text reader and introduce CLIP4STR, a simple yet effective STR method built upon image and text encoders of CLIP. It has two encoder-decoder branches: a visual branch and a cross-modal branch. The visual branch provides an initial prediction based on the visual feature, and the cross-modal branch refines this prediction by addressing the discrepancy between the visual feature and text semantics. To fully leverage the capabilities of both branches, we design a dual predict-and-refine decoding scheme for inference. We scale CLIP4STR in terms of the model size, pre-training data, and training data, achieving state-of-the-art performance on 13 STR benchmarks. Additionally, a comprehensive empirical study is provided to enhance the understanding of the adaptation of CLIP to STR. Our method establishes a simple yet strong baseline for future STR research with VLMs.

==> tables/tab-cross-modal.tex <==
\begin{table}[!t]
    \centering
    % \setlength\tabcolsep{2pt}
    \caption{The importance of cross-modal branch.
    The text length is the sequence length of the text encoder.
    }
    \scalebox{0.66}{
    \begin{tabular}{cc|ccccc}
    \toprule
    cross-modal & text length & IC15 & SVTP & CUTE & HOST & COCO   \\
    \midrule
    \xmark & \xmark & 90.3 & 97.1 & \textbf{99.7} & 76.3 & 80.9   \\

    \cmark & 16 & \textbf{90.6} & \textbf{97.2} & 99.3 & \textbf{77.5} & \textbf{81.1}  \\
    \midrule

    \cmark & 12 & 90.5 & 97.1 & 99.0 & 76.2 & 80.9  \\

    \cmark & 16 & \textbf{90.6} & \textbf{97.2} & 99.3 & \textbf{77.5} & 81.1  \\

    \cmark & 20 & 90.6 & 96.3 & 98.6 & 75.9 & \textbf{81.2}  \\
    \bottomrule
  \end{tabular}}
  \label{tab:cross-modal}
\end{table}
